A fast score-based search algorithm for maximal ancestral graphs using entropy

\emph{Maximal ancestral graph} (MAGs) is a class of graphical model that extend the famous \emph{directed acyclic graph} in the presence of latent confounders. Most score-based approaches to learn the unknown MAG from empirical data rely on BIC score which suffers from instability and heavy computations. We propose to use the framework of imsets \citep{studeny2006probabilistic} to score MAGs using empirical entropy estimation and the newly proposed \emph{refined Markov property} \citep{hu2023towards}. Our graphical search procedure is similar to \citet{claassen2022greedy} but improved from our theoretical results. We show that our search algorithm is polynomial in number of nodes by restricting degree, maximal head size and number of discriminating paths. In simulated experiment, our algorithm shows superior performance compared to other state of art MAG learning algorithms.

==> Shortcuts2-0-2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Packages                                  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{amsmath, amsfonts, amsthm, amssymb, bbm, bm}
\usepackage{mathrsfs}
\usepackage{centernot}
%\usepackage{euscript}
\usepackage{enumerate}
%\usepackage{calligra}
\usepackage{tabularx}
\usepackage{multicol}
\usepackage{multirow}
%\usepackage{relsize}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Symbols                                   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\Pr}{\mathbb{P}}
%\newcommand{\E}{\scalebox{1.1}{$\mathbb{E}$}}
\newcommand{\E}{\mathbb{E}}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\Corr}{Corr}
\newcommand{\Ind}{\mathbbm{1}}

\newcommand{\reals}{\mathbb{R}}

\DeclareMathOperator{\expit}{expit}
\DeclareMathOperator{\logit}{logit}

\newcommand{\G}{\mathcal{G}}
\newcommand{\X}{\mathfrak{X}}

\DeclareMathOperator{\ing}{ing}
\DeclareMathOperator{\diag}{diag}

\DeclareMathOperator{\tail}{tail}
\DeclareMathOperator{\patail}{pa-tail}
\DeclareMathOperator{\distail}{dis-tail}
\DeclareMathOperator{\pa}{pa}
\DeclareMathOperator{\ch}{ch}
\DeclareMathOperator{\nei}{ne}
\DeclareMathOperator{\bd}{bd}
\DeclareMathOperator{\spo}{sp}
\DeclareMathOperator{\an}{an}
\DeclareMathOperator{\ant}{ant}
\DeclareMathOperator{\un}{un}
\DeclareMathOperator{\dir}{dir}
\DeclareMathOperator{\dec}{de}
\DeclareMathOperator{\barren}{barren}
\DeclareMathOperator{\sterile}{sterile}
\DeclareMathOperator{\dis}{dis}
\DeclareMathOperator{\sib}{sib}
\DeclareMathOperator{\nhd}{nhd}
\DeclareMathOperator{\nd}{nd}
\DeclareMathOperator{\mbl}{mb}
\DeclareMathOperator{\forb}{forb}
\DeclareMathOperator{\cn}{cn}

\DeclareMathOperator{\pre}{pre}

\DeclareMathOperator{\Do}{\it do}
\newcommand{\cmid}{\,|\,}

\newcommand{\lrarr}{\leftrightarrow}
\newcommand{\sto}{\mathbin{*\mkern -8mu\to}}
\newcommand{\getss}{\mathbin{\gets\mkern -8mu*}}

\newcommand{\sun}{\mathbin{*\mkern -8mu-}}
\newcommand{\uns}{\mathbin{-\mkern -8mu*}}
\newcommand{\suns}{\mathbin{*\mkern -8mu-\mkern -8mu*}}
\newcommand{\cto}{\mathbin{\circ\!\!\to}}
\newcommand{\getsc}{\mathbin{\gets\!\!\circ}}
\newcommand{\cceg}{\mathbin{\circ\mkern -3.5mu\mathbin{-}}\mkern -3.5mu\circ}
\newcommand{\cseg}{\mathbin{\circ\!\!-\mkern -8mu*}}
\newcommand{\sceg}{\mathbin{*\mkern -8mu-\!\!\circ}}
\newcommand{\cun}{\mathbin{\circ\mkern -3.5mu-}}
\newcommand{\unc}{\mathbin{-\mkern -3.5mu\circ}}
%\newcommand{\lrarr}{\leftrightarrow}
%\newcommand{\sto}{\mathbin{*\mkern -8mu\to}}
%\newcommand{\getss}{\gets\mkern -8mu*}
%\newcommand{\sun}{*\mkern -8mu-}
%\newcommand{\uns}{-\mkern -8mu*}
%\newcommand{\suns}{*\mkern -8mu-\mkern -8mu*}
%\newcommand{\cto}{\circ\!\!\to}
%\newcommand{\getsc}{\gets\!\!\circ}
%\newcommand{\cceg}{\circ\!\!\mathbin{-}\mkern -4mu\circ}
%\newcommand{\cseg}{\circ\!\!-\mkern -8mu*}
%\newcommand{\sceg}{*\mkern -8mu-\!\!\circ}
%\newcommand{\cun}{\circ\!\!-}
%\newcommand{\unc}{-\!\!\circ}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Symbols                                   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\simiid}{\stackrel{\mbox{\tiny{i.i.d.}}}{\sim}}
\newcommand{\simap}{\stackrel{\mbox{approx}}{\sim}}

% Forms of convergence
\newcommand{\tend}{\longrightarrow}
%\newcommand{\tendD}{\xrightarrow{\mathcal{D}}}
\newcommand{\tendD}{\stackrel{\mathcal{D}}{\longrightarrow}}
\newcommand{\tendd}{\stackrel{d}{\longrightarrow}}
%\newcommand{\tendp}{\xrightarrow{p}}
\newcommand{\tendp}{\stackrel{p}{\longrightarrow}}
%\newcommand{\tendas}{\xrightarrow{\mbox{\tiny{a.s.}}}}
\newcommand{\tendas}{\stackrel{\mbox{\tiny{a.s.}}}{\longrightarrow}}
\newcommand{\tendL[1]}{\xrightarrow{L_{#1}}}

\newcommand{\ntend}{\nrightarrow}
\newcommand{\ntendD}{\centernot{\xrightarrow{\mathcal{D}}}}
\newcommand{\ntendp}{\centernot{\xrightarrow{\mathbb{P}}}}
\newcommand{\ntendas}{\centernot{\xrightarrow{\mbox{\tiny{a.s.}}}}}
\newcommand{\ntendL[1]}{\centernot{\xrightarrow{L_{#1}}}}

\newcommand{\eqD}{\stackrel{\mathcal{D}}{=}}
\newcommand{\eqas}{\stackrel{\mbox{\tiny\rm a.s.}}{=}}

\newcommand{\T[1]}{{#1}^T}

\newcommand\indep{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

%\newcommand{\nindep}{\indep\!\!\!\!\!\!\setminus\;\;}
\newcommand{\nindep}{\centernot{\indep}}

\newcommand{\CI}[3]{#1 \indep #2 \; | \; #3}
\newcommand{\GS}[3]{#1 \perp #2 \; | \; #3}

\newcommand{\rbow}{\mathbin{\begin{tikzpicture}[baseline] 
\draw[<->] (0pt,.3ex) -- (2ex,.3ex);
\draw[->] (0pt,1ex) -- (2ex,1ex);
\end{tikzpicture}}}

\newcommand{\lbow}{\mathbin{\begin{tikzpicture}[baseline] 
\draw[<->] (0pt,.3ex) -- (2ex,.3ex);
\draw[<-] (0pt,1ex) -- (2ex,1ex);
\end{tikzpicture}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Theorems                                  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{lem}{Lemma}[section]
\newtheorem{thm}[lem]{Theorem}
\newtheorem{prop}[lem]{Proposition}
\newtheorem{cor}[lem]{Corollary}
\newtheorem{conj}[lem]{Conjecture}
\theoremstyle{definition}
\newtheorem{dfn}[lem]{Definition}
%\theoremstyle{remark}
\newtheorem{rmk}[lem]{Remark}
\newtheorem{exm}[lem]{Example}
\newtheorem{alg}[lem]{Algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Environments                              %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\benum}{\begin{enumerate}}
\newcommand{\eenum}{\end{enumerate}}

\newcommand{\bitem}{\begin{itemize}}
\newcommand{\eitem}{\end{itemize}}

\newcommand{\barr}{\begin{array}}
\newcommand{\earr}{\end{array}}

\newcommand{\bmat}{\begin{pmatrix}}
\newcommand{\emat}{\end{pmatrix}}

\newcommand{\blist}{\renewcommand{\labelenumi}{\textbf{\arabic{enumi}}.} \begin{enumerate}}
\newcommand{\elist}{\end{enumerate} \renewcommand{\labelenumi}{\arabic{enumi}.}}

%\newcommand{\mb}{\mathbf}
\newcommand{\bs}{\boldsymbol}

\def\bal#1\eal{\begin{align*}#1\end{align*}}

\newcommand{\stk}[2]{\mathsmaller{\begin{smallmatrix}#1 \\ #2\end{smallmatrix}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Indents                                   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setlength{\parindent}{0pt}
\setlength{\parskip}{6pt}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TikZ Commands                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{tikz}
\usetikzlibrary{shapes, arrows, arrows.meta, calc, positioning}


% nodes
\tikzset{nv/.style={circle, color=red, fill=red, inner sep=0.5mm}}
\tikzset{rv/.style={circle, draw, thick, minimum size=6.5mm, inner sep=0.5mm}}
\tikzset{fv/.style={rectangle, draw, thick, minimum size=6mm, inner sep=0.5mm}}
\tikzset{lv/.style={circle, color=red, fill=gray!30, draw, thick, minimum size=6.5mm, inner sep=0.5mm}}
\tikzset{rve/.style={ellipse, draw, thick, minimum size=6.5mm, inner sep=0.5mm}}

% nodes for slides
\tikzset{rvs/.style={circle, draw, thick, minimum size=5.5mm, inner sep=0.5mm}}
\tikzset{fvs/.style={rectangle, draw, thick, minimum size=5mm, inner sep=0.5mm}}
\tikzset{lvs/.style={circle, color=red, fill=gray!30, draw, thick, minimum size=5.5mm, inner sep=0.5mm}}
\tikzset{rves/.style={ellipse, draw, thick, minimum size=5.5mm, inner sep=0.5mm}}

% edges
\tikzset{deg/.style={->, very thick, color=blue}}
\tikzset{sdeg/.style={*->, very thick, color=blue}}
\tikzset{degl/.style={->, very thick, color=red}}
\tikzset{beg/.style={<->, very thick, color=red}}
%\pgfarrowsdeclare{os}{os}{}{$\circ$} 
\tikzset{cdeg/.style={{Circle[length=+2pt 2.5,width=+2pt 2.5, fill=none]}->, very thick, color=blue}}
\tikzset{cceg/.style={{Circle[length=+2pt 2.5,width=+2pt 2.5, fill=none]}-{Circle[length=+2pt 2.5,width=+2pt 2.5, fill=none]}, very thick}}
\tikzset{uceg/.style={{Circle[length=+2pt 2.5,width=+2pt 2.5, fill=none]}-, very thick}}
\tikzset{ueg/.style={very thick}}




